A Formula for the Jones-Wenzl Projections

I present a method of calculating the coefficients appearing in the Jones-Wenzl projections in the Temperley-Lieb algebras. It essentially repeats the approach of Frenkel and Khovanov published in 1997. I wrote this note mid-2002, not knowing about their work, but then set it aside upon discovering their article. Recently I decided to dust it off and place it on the arXiv --- hoping the self-contained and detailed proof I give here may be useful. It's also been cited a number of times, so I thought it best to give it a permanent home. The proof is based upon a simplification of the Wenzl recurrence relation. I give an example calculation, and compare this method to the formula announced by Ocneanu and partially proved by Reznikoff. I also describe certain moves on diagrams which modify their coefficients in a simple way.

==> diagram.tex <==
\xybox{
(1.5,0);(28.5,18) **i@{-},(3,18);(3,0)  **\crv{(3,5.4)&(3,12.6)},
(6,18);(12,0)  **\crv{(6,5.4)&(12,12.6)},
(9,18);(15,0)  **\crv{(9,5.4)&(15,12.6)},
(12,18);(21,18)  **\crv{(12,12.6)&(21,12.6)},
(15,18);(18,18)  **\crv{(15,16.2)&(18,16.2)},
(24,18);(27,18)  **\crv{(24,16.2)&(27,16.2)},
(27,0);(18,0)  **\crv{(27,5.4)&(18,5.4)},
(24,0);(21,0)  **\crv{(24,1.8)&(21,1.8)},
(9,0);(6,0)  **\crv{(9,1.8)&(6,1.8)},
}

==> generated-diagrams-template.tex <==
\newcommand{\xyTLFiveTwentySix}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[5,26],DiagramHeight->28],DiagramHeight->28]
}
\newcommand{\xyTLFiveTwentyFiveTimesTLFiveTwelve} { %-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TemperleyLiebXyBox[TL[5,25],DiagramHeight->16],TemperleyLiebXyBox[TL[5,12],DiagramHeight->12]}],DiagramHeight->28]
}
\newcommand{\xyMultiplicativeGeneratorFiveOne}{ %-def TemperleyLiebXyBox[MultiplicativeGenerator[5,1]]
}
\newcommand{\xyMultiplicativeGeneratorFiveTwo}{ %-def TemperleyLiebXyBox[MultiplicativeGenerator[5,2]]
}
\newcommand{\xyMultiplicativeGeneratorFiveThree}{ %-def TemperleyLiebXyBox[MultiplicativeGenerator[5,3]]
}
\newcommand{\xyMultiplicativeGeneratorFiveFour}{ %-def TemperleyLiebXyBox[MultiplicativeGenerator[5,4]]
}
\newcommand{\xyJonesWenzlIdempotentSixPlusOne}[1]{%-def VerticallyCenterXyBox[TensorXyBoxes[{TextAcrossDottedStrandsXyBox[#1,3,2],TemperleyLiebXyBox[TL[1,1]]}],DiagramHeight->18]
}
\newcommand{\xyJonesWenzlIdempotentSeven}[1]{%-def VerticallyCenterXyBox[TextAcrossDottedStrandsXyBox[#1,3,3],DiagramHeight->18]
}
\newcommand{\xyWenzlRecurrenceLastTermSixPlusOne}[1]{%-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TensorXyBoxes[{TextAcrossDottedStrandsXyBox[#1,3,2],TemperleyLiebXyBox[TL[1,1]]}],TensorXyBoxes[{TemperleyLiebXyBox[TL[3,1],DiagramHeight->4],"\xybox{*i"<>TemperleyLiebXyBox[TL[1,1],DiagramHeight->4]<>"}",TemperleyLiebXyBox[MultiplicativeGenerator[3,2],DiagramHeight->4]}],TensorXyBoxes[{TextAcrossDottedStrandsXyBox[#1,3,2],TemperleyLiebXyBox[TL[1,1]]}]}],DiagramHeight->40]
}
\newcommand{\xySingleRightCupSixOne}{%-def TemperleyLiebXyBox[SingleRightCup[6,1],StringSpacing->3,DiagramHeight->18]
}
\newcommand{\xySingleRightCupSixTwo}{%-def TemperleyLiebXyBox[SingleRightCup[6,2],StringSpacing->3,DiagramHeight->18]
}
\newcommand{\xySingleRightCupSixThree}{%-def TemperleyLiebXyBox[SingleRightCup[6,3],StringSpacing->3,DiagramHeight->18]
}
\newcommand{\xySingleRightCupSixFour}{%-def TemperleyLiebXyBox[SingleRightCup[6,4],StringSpacing->3,DiagramHeight->18]
}
\newcommand{\xySingleRightCupSixFive}{%-def TemperleyLiebXyBox[SingleRightCup[6,5],StringSpacing->3,DiagramHeight->18]
}
\newcommand{\xySingleRightCupSixSix}{%-def TemperleyLiebXyBox[SingleRightCup[6,6],StringSpacing->3,DiagramHeight->18]
}
\newcommand{\xyMultiplicativeGeneratorSixFiveTimesGFiveThree}{%-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TemperleyLiebXyBox[MultiplicativeGenerator[6,5],DiagramHeight->9],TensorXyBoxes[{TemperleyLiebXyBox[SingleRightCup[5,3],DiagramHeight->9],TemperleyLiebXyBox[TL[1,1],DiagramHeight->9]}]}],DiagramHeight->18]
}
\newcommand{\xyGSixThree}{%-def VerticallyCenterXyBox[TemperleyLiebXyBox[SingleRightCup[6,3],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyCaseOne}{%-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TensorXyBoxes[{"\xybox{*"<>TextAcrossStrandsXyBox["h",4,DiagramHeight->12]<>",(6,2.4);(9,2.4) **h\crv{(6,4)&(9,4)}}",TemperleyLiebXyBox[TL[1,1],DiagramHeight->12]}],TemperleyLiebXyBox[SingleRightCup[5,2],DiagramHeight->12]}],DiagramHeight->24]
}
\newcommand{\xyCaseTwo}{%-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TensorXyBoxes[{"\xybox{*"<>TextAcrossStrandsXyBox["h",4,DiagramHeight->12]<>",(9,2.4);(12,2.4) **h\crv{(9,4)&(12,4)}}",TemperleyLiebXyBox[TL[1,1],DiagramHeight->12]}],TemperleyLiebXyBox[SingleRightCup[5,2],DiagramHeight->12]}],DiagramHeight->24]
}
\newcommand{\xyCaseThree}{%-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TensorXyBoxes[{TextAcrossStrandsXyBox["{\Id}",4,DiagramHeight->12],TemperleyLiebXyBox[TL[1,1],DiagramHeight->12]}],TemperleyLiebXyBox[SingleRightCup[5,2],DiagramHeight->12]}],DiagramHeight->24]
}
\newcommand{\xyTLSixSeventyNine}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[6,79],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLSixEightyOneAndCap}{ %-def VerticallyCenterXyBox[TensorXyBoxes[{TemperleyLiebXyBox[TL[6,81],DiagramHeight->18],SingleCapXyBox[DiagramHeight->18]}],DiagramHeight->18]
}
\newcommand{\xyTLSixSeventyNineTimesGSevenThree}{%-def VerticallyCenterXyBox[ConcatenateXyBoxes[{TensorXyBoxes[{TemperleyLiebXyBox[TL[6,79],DiagramHeight->13],TemperleyLiebXyBox[TL[1,1],DiagramHeight->13]}],TemperleyLiebXyBox[SingleRightCup[7,3],DiagramHeight->13]}],DiagramHeight->26]
}
\newcommand{\xyTLSevenTwoHundredAndSixtyFive}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[7,265],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLFiveEight}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[5,8],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyFoldDownTLFiveEight}{ %-def VerticallyCenterXyBox[TensorXyBoxes[{TemperleyLiebXyBox[TL[4,3],DiagramHeight->8,StringSpacing->1.5],SingleCapXyBox[DiagramHeight->8,StringSpacing->1.5]}],DiagramHeight->8]
}
\newcommand{\xyTLFourTwo}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[4,2],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLFourThree}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[4,3],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLThreeOne}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,1],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLThreeTwo}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,2],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLThreeThree}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,3],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLThreeFour}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,4],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLThreeFive}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,5],DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyFoldDownTLFourTwo}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBoxWithOmits[TL[5,3],{4,5},DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyFoldDownTLFourThree}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBoxWithOmits[TL[5,4],{4,5},DiagramHeight->8,StringSpacing->1.5],DiagramHeight->8]
}
\newcommand{\xyTLFiveEightFullSize}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[5,8],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyCapFormTLFiveEight}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBoxWithOmits[TL[10,16762],Range[10],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLMoveInitial}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[10,16713],DiagramHeight->22],DiagramHeight->22]
}
\newcommand{\xyTLMoveFinalOne}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[10,16716],DiagramHeight->22],DiagramHeight->22]
}
\newcommand{\xyTLMoveFinalTwo}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[10,16727],DiagramHeight->22],DiagramHeight->22]
}
\newcommand{\xyTLThreeOneFullSize}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,1],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLThreeTwoFullSize}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,2],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLThreeThreeFullSize}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,3],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLThreeFourFullSize}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,4],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xyTLThreeFiveFullSize}{ %-def VerticallyCenterXyBox[TemperleyLiebXyBox[TL[3,5],DiagramHeight->18],DiagramHeight->18]
}
\newcommand{\xySampleN} { %-def VerticallyCenterXyBox[TemperleyLiebXyBox[\[ScriptCapitalN][19,4,7,4,7],DiagramHeight->18],DiagramHeight->18]
}

